A second order primal-dual method for nonsmooth convex composite optimization

We develop a second order primal-dual method for optimization problems in which the objective function is given by the sum of a strongly convex twice differentiable term and a possibly nondifferentiable convex regularizer. After introducing an auxiliary variable, we utilize the proximal operator of the nonsmooth regularizer to transform the associated augmented Lagrangian into a function that is once, but not twice, continuously differentiable. The saddle point of this function corresponds to the solution of the original optimization problem. We employ a generalization of the Hessian to define second order updates on this function and prove global exponential stability of the corresponding differential inclusion. Furthermore, we develop a globally convergent customized algorithm that utilizes the primal-dual augmented Lagrangian as a merit function. We show that the search direction can be computed efficiently and prove quadratic/superlinear asymptotic convergence. We use the $\ell_1$-regularized model predictive control problem and the problem of designing a distributed controller for a spatially-invariant system to demonstrate the merits and the effectiveness of our method.

==> MakCommands.tex <==
%%%%%% Makan's commands %%%%%%%%%%%%

%\newcommand{\MakanWork}{/Users/Makan/Research/Mak}
%\newcommand{\WorkPapers}{\MakanWork/Mak_Papers}
%\newcommand{\WorkPresent}{\MakanWork/Presentations}

%% The folloing setlength commands were
%% taken out when writting final version of
%% Nyquist paper, 8th Sept 2005.
%\setlength{\textwidth}{6.5 in}
%\setlength{\oddsidemargin}{0 in}
%\setlength{\evensidemargin}{0 in}


%%% text

\newcommand{\etal}{{\em et al. }}

%%% Commands

\newcommand{\non}{\nonumber}

\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bes}{\begin{equation*}}
\newcommand{\ees}{\end{equation*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}	
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}
\newcommand{\br}{\begin{remark}}
\newcommand{\er}{\end{remark}}
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bp}{\begin{proof}}
\newcommand{\ep}{\end{proof}}

%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
%\newcommand{\beqs}{\begin{equation*}}
%\newcommand{\eeqs}{\end{equation*}}
%\newcommand{\beqn}{\begin{eqnarray}}
%\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\beqns}{\begin{eqnarray*}}	%old; use \beas
\newcommand{\eeqns}{\end{eqnarray*}}		%old; use \eeas
\newcommand{\bct}{\begin{center}}		%old; use \bc
\newcommand{\ect}{\end{center}}			%old; use \ec
\newcommand{\benum}{\begin{enumerate}}	%old; use \ben
\newcommand{\eenum}{\end{enumerate}}		%old; use \een

% spacings and separators

\newcommand{\linespace}{\\[-0.1in]}

\newcommand{\hsp}{\hspace{-0.1in}} 
\newcommand{\hof}{\hspace{-0.05in}} 

\newcommand{\smallblock}{\hfill \rule{1ex}{1ex}}		
\newcommand{\bigblock}{\hfill \rule{1.3ex}{1.3ex}}	

%\newcommand{\bigbox}{\hfill $\Box$}
\newcommand{\boxend}{\hfill $\square$}
\newcommand{\blockend}{\hfill $\blacksquare$}


%%% Notations

\newcommand{\scr}{\mathscr}
\newcommand{\eus}{\EuScript}

\newcommand{\Ups}{\Upsilon}
\newcommand{\lam}{\lambda}
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}
\newcommand{\vappa}{\varkappa}
\newcommand{\vhi}{\varphi}
\newcommand{\veta}{\vartheta}

\newcommand{\CRHP}{\mathbb{C}^{+}}
\newcommand{\OLHP}{\mathbb{C}^{-}}

% special letters

\newcommand{\ii}{\mathrm{i}}    % \ii = sqrt(-1)
\newcommand{\jj}{\mathrm{j}}    % \jj = sqrt(-1)
\newcommand{\dd}{\mathrm{d}}    % as in the differential dx 
\newcommand{\expo}{\mathrm{e}}    % e = 2.71... 

% sets

\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbU}{\mathbb{U}}

\newcommand{\sX}{\mathsf{X}}
\newcommand{\sM}{\mathsf{M}}

\newcommand{\eX}{\eus{X}}  % Space X where the state resides at any time t 
\newcommand{\eU}{\eus{U}}   % Space U where the input resides at any time t
\newcommand{\eY}{\eus{Y}}   % Space Y where the output resides at any time t

\newcommand{\BddX}{\scr{B}(\eX)}
\newcommand{\BcompX}{\scr{B}_\infty(\eX)}
\newcommand{\BtwoX}{\scr{B}_2(\eX)}
\newcommand{\BoneX}{\scr{B}_1(\eX)}
\newcommand{\BzeroX}{\scr{B}_0(\eX)} %change to \Bcomp

\newcommand{\BddY}{\scr{B}(\eY)}
\newcommand{\BcompY}{\scr{B}_\infty(\eY)}
\newcommand{\BtwoY}{\scr{B}_2(\eY)}
\newcommand{\BoneY}{\scr{B}_1(\eY)}

\newcommand{\Bdd}{\scr{B}(\ell^2)}
\newcommand{\Bcomp}{\scr{B}_\infty(\ell^2)}
\newcommand{\Btwo}{\scr{B}_2(\ell^2)}
\newcommand{\Bone}{\scr{B}_1(\ell^2)}
\newcommand{\Bzero}{\scr{B}_0(\ell^2)} %change to \Bcomp

\newcommand{\LlO}{L_{\ell^2}^2[0,\Omega]}

\newcommand{\LlBarT}{L_{\ell^2}^2(\overline{\Theta})}
\newcommand{\LlT}{L_{\ell^2}^2(\Theta)}
\newcommand{\BarT}{\overline{\Theta}}
% The above had conflict with letter "O" at the end.
% Has been changed to "T". The original form was as follows:
%\newcommand{\LlBarO}{L_{\ell^2}^2(\overline{\Theta})}
%\newcommand{\LlO}{L_{\ell^2}^2(\Theta)}
%\newcommand{\BarO}{\overline{\Theta}}

\newcommand{\dom}{\mathscr{D}}

\newcommand{\Zee}{\scr{Z}} 

\newcommand{\Cone}{\scr{C}}  	% cone causal systems

\newcommand{\Stab}{\scr{S}}  	% stable systems
\newcommand{\unStab}{\scr{S}^\perp}  	% unstable systems

\newcommand{\fD}{\frak{D}}
\newcommand{\fDs}{\frak{D}^\theta}    


%%% Functions and Operators

\newcommand{\Adv}{\mathbb{A}}  %Advection/Perron-Frobenius inf-generator
\newcommand{\PF}{\mathbb{P}}  %Perron-Frobenius operator
\newcommand{\PFh}{\hat{\mathbb{P}}}  %Perron-Frobenius operator
\newcommand{\Badv}{\mathbb{B}}  %Advection input operator

% dots

\newcommand{\Vdot}{\dot{V}}
\newcommand{\xdot}{\dot{x}}
\newcommand{\rhodot}{\dot{\rho}}

% bars

\newcommand{\rhobar}{\bar{\rho}}
\newcommand{\mubar}{\bar{\mu}}

% calculus

\newcommand{\ident}{\equiv} 

\newcommand{\grad}{\nabla}  %gradient
\newcommand{\curl}{\mathrm{curl}}  %gradient
\newcommand{\diverge}{\mathrm{div}}  %divergence
\newcommand{\laplace}{\Delta}  %laplacian

% matrix stuff, etc

\newcommand{\enma}[1]   {\ensuremath{#1}}
\newcommand{\tr}        {\enma{\mathrm{tr}}}
\newcommand{\diag}      {\enma{\mathrm{diag}}}
\newcommand{\toep}      {\enma{\mathrm{toep}}}
\newcommand{\Ker}       {\enma{\mathrm{Ker}}}
\newcommand{\trace}     {\enma{\mathrm{trace}}}
\newcommand{\co}        {\enma{\mathrm{co}}}
\newcommand{\col}       {\enma{\mathrm{col}}}
\newcommand{\rad}       {\enma{\mathrm{rad}}}
\newcommand{\rank}     {\enma{\mathrm{rank}}}
\newcommand{\blockdiag} {\enma{\mathrm{blockdiag}}}
\newcommand{\eig}       {\enma{\mathrm{eig}}}
\newcommand{\sgn}       {\enma{\mathrm{sgn}}}
\newcommand{\residue}   {\enma{\mathrm{Res}}}
\newcommand{\re}        {\enma{\mathrm{Re}}}
\newcommand{\im}        {\enma{\mathrm{Im}}}
\newcommand{\ess}        {\enma{\mathrm{ess}}}

% hats

\newcommand{\vh}{\hat{v}}
\newcommand{\wh}{\hat{w}}
\newcommand{\ph}{\hat{\psi}}
\newcommand{\phh}{\hat{\phi}}
\newcommand{\gih}{\hat{g}}
\newcommand{\uh}{\hat{u}}
\newcommand{\xh}{\hat{x}}
\newcommand{\yh}{\hat{y}}
\newcommand{\zh}{\hat{z}}

\newcommand{\Ah}{\hat{A}}
\newcommand{\Bh}{\hat{B}}
\newcommand{\Ch}{\hat{C}}
\newcommand{\Dh}{\hat{D}}
\newcommand{\Eh}{\hat{E}}
\newcommand{\Gh}{\hat{G}}
\newcommand{\Ih}{\hat{I}}
\newcommand{\Kh}{\hat{K}}
\newcommand{\Qh}{\hat{Q}}
\newcommand{\Rh}{\hat{R}}
\newcommand{\Sh}{\hat{S}}
\newcommand{\Th}{\hat{T}}

% theta index

\newcommand{\us}{u_\theta}
\newcommand{\vs}{v_\theta}
\newcommand{\ys}{y_\theta}
\newcommand{\pss}{\psi_\theta}
\newcommand{\phs}{\phi_\theta}

\newcommand{\As}{{\cal A}_\theta}
\newcommand{\Bs}{{\cal B}_\theta}
\newcommand{\Cs}{{\cal C}_\theta}
\newcommand{\Ds}{{\cal D}_\theta}
\newcommand{\Es}{{\cal E}_\theta}
\newcommand{\Gs}{{\cal G}_\theta}
\newcommand{\Ks}{{\cal K}_\theta}
\newcommand{\Ps}{{\cal P}_\theta}
\newcommand{\Qs}{{\cal Q}_\theta}
\newcommand{\Rs}{{\cal R}_\theta}
\newcommand{\Ss}{{\cal S}_\theta}

\newcommand{\Acls}{{\cal A}_{\theta}^\cl}
\newcommand{\Gcls}{{\cal G}_{\theta}^\cl}

% \vartheta index

\newcommand{\Gvs}{{\cal G}_\vartheta}
\newcommand{\Avs}{{\cal A}_\vartheta}
\newcommand{\Bvs}{{\cal B}_\vartheta}
\newcommand{\Cvs}{{\cal C}_\vartheta}

\newcommand{\Aclvs}{{\cal A}_{\vartheta}^\cl}

% caligraphic/script

\newcommand{\A}{{\cal A}}
\newcommand{\B}{{\cal B}}
\newcommand{\C}{{\cal C}}
\newcommand{\D}{{\cal D}}
\newcommand{\E}{{\cal E}}
\newcommand{\F}{{\cal F}}
\newcommand{\G}{{\cal G}}
\newcommand{\eicH}{{\cal H}}
\newcommand{\I}{{\cal I}}
\newcommand{\K}{{\cal K}}
\newcommand{\eL}{{\cal L}}
\newcommand{\M}{{\cal M}}
\newcommand{\Pee}{{\cal P}}
\newcommand{\Q}{{\cal Q}}
\newcommand{\R}{{\cal R}}
\newcommand{\eS}{{\cal S}}
\newcommand{\X}{{\cal X}}
\newcommand{\Z}{{\cal Z}}

\newcommand{\Fs}{{\cal F}}
\newcommand{\Is}{{\cal I}}

\newcommand{\Acl}{\A^\cl}
\newcommand{\Gcl}{\G^\cl}

\newcommand{\Atilde}{\widetilde{\cal A}}
\newcommand{\Btilde}{\widetilde{\cal B}}
\newcommand{\Ctilde}{\widetilde{\cal C}}
\newcommand{\Gtilde}{\widetilde{\cal G}}

% frak

\newcommand{\fRs}{\frak{R}_\theta}
\newcommand{\fGs}{\frak{G}_\theta}
\newcommand{\fAs}{\frak{A}_\theta}
\newcommand{\fBs}{\frak{B}_\theta}
\newcommand{\fCs}{\frak{C}_\theta}
\newcommand{\fEs}{\frak{E}_\theta}
\newcommand{\fFs}{\frak{F}}
\newcommand{\fIs}{\frak{I}}

% mathtt

\newcommand{\tRs}{\mathtt{R}_\theta}
\newcommand{\tGs}{\mathtt{G}_\theta}
\newcommand{\tAs}{\mathtt{A}_\theta}
\newcommand{\tBs}{\mathtt{B}_\theta}
\newcommand{\tCs}{\mathtt{C}_\theta}
\newcommand{\tEs}{\mathtt{E}_\theta}
\newcommand{\tPs}{\mathtt{P}_\theta}
\newcommand{\tQs}{\mathtt{Q}_\theta}
\newcommand{\tFs}{\mathtt{F}}
\newcommand{\tIs}{\mathtt{I}}

% roman

\newcommand{\rX}{{\rm X}}
\newcommand{\rV}{{\rm V}}

\newcommand{\ru}{{\rm u}}
\newcommand{\ruh}{\hat{\rm u}}
\newcommand{\ry}{{\rm y}}
\newcommand{\ryh}{\hat{\rm y}}

\newcommand{\rG}{{\rm G}}
\newcommand{\rGs}{{\rm G}_\theta}
\newcommand{\rGh}{\hat{\rm G}}
\newcommand{\rS}{{\rm S}}
\newcommand{\rSh}{\hat{\rm S}}

\newcommand{\rA}{{\rm A}}
\newcommand{\rB}{{\rm B}}
\newcommand{\rC}{{\rm C}}
\newcommand{\rD}{{\rm D}}

% underline

\newcommand{\Gu}{\underline{G}}
\newcommand{\Gus}{\underline{\cal G}_\theta}
\newcommand{\rGu}{\underline{\rm G}}
\newcommand{\Ru}{\underline{R}}
\newcommand{\rSu}{\underline{\rm S}}
\newcommand{\Su}{\underline{S}}

% miscellaneous

\newcommand{\one}{\mathbbmtt{1}}  % need to add \usepackage{bbm} at beginning

\newcommand{\LMA}{\scr{L}_{{\cal A}_\theta}}
\newcommand{\RMAs}{\scr{R}_{{\cal A}_\theta^*}}

\newcommand{\Sols}{\mathbf{S_{\theta}^\ol}}
\newcommand{\Scls}{\mathbf{S_{\theta}^\cl}}

\newcommand{\cM}{{\cal M}}
\newcommand{\Ms}{\scr{M}_\theta}
\newcommand{\expect}{\scr{E}}
\newcommand{\proj}{\Pi}

\newcommand{\vsnot}{v_{\theta_0}}
\newcommand{\Gsnot}{{\cal G}_{\theta_0}}

% running variables

\newcommand{\Aok}{A_0(k)}
\newcommand{\Adot}{A_0(\,\cdot\,)}

\newcommand{\pardot}{(\,\cdot\,)}
\newcommand{\spacedot}{\,\cdot\,}



%%% sub- & super-scripts

\newcommand{\ol}{\text{o}}
\newcommand{\cl}{\text{cl}}
\newcommand{\maxim}{\text{max}}
\newcommand{\minim}{\text{min}}
\newcommand{\res}{\text{res}}
\newcommand{\spa}{\text{sp}}
\newcommand{\opt}{\text{opt}}
\newcommand{\cen}{\text{cen}}
\newcommand{\param}{\text{par}}
\newcommand{\outter}{\text{out}}
\newcommand{\inner}{\text{in}}
\newcommand{\stab}{\text{st}}		% stable part
\newcommand{\unstab}{\text{un}}		% unstable part

\newcommand{\Sigmap}{\Sigma_{\text{p}}}

\newcommand{\sigmax}{\sigma_\maxim}
\newcommand{\sigmin}{\sigma_\minim}
\newcommand{\lamax}{\lambda_\maxim}
\newcommand{\lamin}{\lambda_\minim}

\newcommand{\lamn}{\lambda_n}
\newcommand{\sign}{\sigma_n}

\newcommand{\lamns}{\lambda_n^\theta}
\newcommand{\signs}{\sigma_n^\theta}



%%% norms

\newcommand{\HS}{{\rm HS}}
\newcommand{\cHt}{{\cal H}^2}   %old; use \Htwo
\newcommand{\Htwo}{{\cal H}^2}   
\newcommand{\cHinf}{{\cal H}^\infty}  %old; use \Hinf
\newcommand{\Hinf}{{\cal H}^\infty}
\newcommand{\cHtsp}{{\cal H}^2_\text{sp}}   %old; use \Htwosp
\newcommand{\Htwosp}{{\cal H}^2_\text{sp}}   
\newcommand{\cHinfsp}{{\cal H}^\infty_\text{sp}}   %old; use \Hinfsp
\newcommand{\Hinfsp}{{\cal H}^\infty_\text{sp}}



%%% Theorems, unified numbering

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{axiom}[theorem]{Axiom}

\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{assumption}{Assumption}

%{ % these settings define remarks and example as parts
%  % of text typeset in upshape (and not italic) fonts.
%\theorembodyfont{\upshape}
%\newtheorem{remark}{Remark}
%\newtheorem{example}{Example}
%}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

%\newenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \hspace*{\fill} \rule{0.5em}{0.5em}}




%%% Array stuff

% Sets uniform spacing for all matrices. To avoid it just comment out
% the renewcommand stuff

\newcommand{\matbegin}{
%       \renewcommand{\baselinestretch}{1.5}
%       \renewcommand{\arraystretch}{0.7}
        \left[
}
\newcommand{\matend}{
        \right]
}



\newcommand{\tbo}[2]{
  \matbegin \begin{array}{c}
       #1 \\ #2
       \end{array} \matend }
\newcommand{\thbo}[3]{
  \matbegin \begin{array}{c}
       #1 \\ #2 \\ #3
       \end{array} \matend }
\newcommand{\obt}[2]{
  \matbegin \begin{array}{cc}
       #1 & #2
       \end{array} \matend }
\newcommand{\obth}[3]{
  \matbegin \begin{array}{ccc}
       #1 & #2 & #3
       \end{array} \matend }
\newcommand{\tbt}[4]{
  \matbegin \begin{array}{cc}
       #1 & #2 \\ #3 & #4
       \end{array} \matend }
\newcommand{\thbt}[6]{
  \matbegin \begin{array}{cc}
       #1 & #2 \\ #3 & #4 \\ #5 & #6
       \end{array} \matend }
\newcommand{\tbth}[6]{
  \matbegin \begin{array}{ccc}
       #1 & #2 & #3\\ #4 & #5 & #6
       \end{array} \matend }
\newcommand{\thbth}[9]{
 \matbegin \begin{array}{ccc}
                #1 & #2 & #3 \\
                #4 & #5 & #6 \\
                #7 & #8 & #9
                \end{array}\matend}
\newcommand{\fbo}[4]{
 \matbegin \begin{array}{c}
                #1 \\ #2 \\ #3 \\ #4
                \end{array}\matend}
\newcommand{\obf}[4]{
 \matbegin \begin{array}{cccc}
                #1 & #2 & #3 & #4
                \end{array}\matend}


\newcommand{\tbtb}[4]{
  \matbegin \begin{array}{cc}  \displaystyle
       #1 &  \displaystyle #2 \\  \displaystyle #3 &  \displaystyle #4
       \end{array} \matend }


\newcommand{\stsp}[4]{  \matbegin \begin{array}{c|c}
       #1 & #2 \\ \hline
       #3 & #4
       \end{array} \matend }

\newcommand{\stsptbth}[6]{  \matbegin \begin{array}{c|cc}
       #1 & #2 & #3\\ \hline
       #4 & #5 & #6
       \end{array} \matend }

\newcommand{\stspthbt}[6]{  \matbegin \begin{array}{c|c}
       #1 & #2 \\ \hline
       #3 & #4 \\
       #5 & #6
       \end{array} \matend }

\newcommand{\stspthbth}[9]{  \matbegin \begin{array}{c|cc}
        #1 & #2 & #3 \\ \hline
        #4 & #5 & #6 \\
        #7 & #8 & #9
       \end{array} \matend }
       
       

\newcommand{\system}[4]{
 \left[
  \begin{array}{c|c}
   #1 & #2 \\
   \hline
   #3 & #4
  \end{array}
 \right]
  }
\newcommand{\systemb}[9]{
 \left[
  \begin{array}{cc|c}
   #1 & #2 & #3   \\
   #4 & #5 & #6   \\
   \hline
   #7 & #8 & #9
  \end{array}
 \right]
  }
\newcommand{\systembd}[9]{
 \left[
  \begin{array}{c|cc}
   #1 & #2 & #3   \\
   \hline
   #4 & #5 & #6   \\
   #7 & #8 & #9
  \end{array}
 \right]
  }


==> Tikz_common_styles.tex <==
%_______________________________________________________________
%
%     Tikz_common_styles
%
%     TikZ styles for drawing block diagrams.
%
%      Roy Smith,  15 July 2014
%
%_______________________________________________________________
\typeout{Reading Tikz styles:  Tikz_common_styles}
%
%   Block diagram styles
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=1.0cm,
                                top color=blue!10, bottom color=blue!10]%
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]%
\tikzstyle{connector} = [->,thick]%
\tikzstyle{line} = [thick]%
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]%
\tikzstyle{guide} = []%
%
%   colours for various blocks
\tikzstyle{deltablock} = [block, top color=red!10, bottom color=red!10]%
\tikzstyle{controlblock} = [block, top color=green!10, bottom color=green!10]%
\tikzstyle{weightblock} = [block, top color=orange!10, bottom color=orange!10]%
\tikzstyle{clpblock} = [block, top color=cyan!10, bottom color=cyan!10]%
%
%  styles for dimming block components.
\tikzstyle{block_dim} = [draw,rectangle,thick,minimum height=2em,minimum width=2em,
                                color=black!15]%
\tikzstyle{sum_dim} = [draw,circle,inner sep=0mm,minimum size=2mm,color=black!15]%
\tikzstyle{connector_dim} = [->,thick,color=black!15]%
%
%    Graph styles
\tikzstyle{smalllabel} = [font=\footnotesize]%
\tikzstyle{axiswidth}=[semithick]%
\tikzstyle{axiscolor}=[color=black!50]%
\tikzstyle{help lines} =[color=blue!40,very thin]%
\tikzstyle{axes} = [axiswidth,axiscolor,<->,smalllabel]%
\tikzstyle{axis} = [axiswidth,axiscolor,->,smalllabel]%
\tikzstyle{tickmark} = [thin,smalllabel]%
\tikzstyle{plain_axes} = [axiswidth,smalllabel]%
\tikzstyle{w_axes} = [axiswidth,->,smalllabel]%
\tikzstyle{m_axes} = [axiswidth,smalllabel]%
\tikzstyle{dataplot} = [thick]%
%
%_______________________________________________________________


==> optalg.tex <==
\input{Tikz_common_styles}%
\noindent%
%   set a filename for externalization
%\tikzsetnextfilename{clp_Ndelta_config}
%
\begin{tikzpicture}[scale=1, auto, >=stealth']

    \small

   % specify with respect to the plant

     \node[clpblock, minimum height=1.25cm, minimum width=1.25cm] (N)  {$G$};

     \node[deltablock, minimum height=1cm, minimum width=1cm, anchor=south]
                      (delta) at ($(N.north) + (0,0.7cm)$) {$\nabla f - mI$};

     \node[deltablock, minimum height=1cm, minimum width=1cm, anchor=south]
                      (delta2) at ($(delta.north) + (0,0.35cm)$) {$\mu\nabla M_{\mu g}$};

     \def\ioOffset{0.25cm}
     \coordinate (Nv) at ($(N.east) + (0,\ioOffset)$);
     \coordinate (Nu) at ($(N.east) - (0,\ioOffset)$);
     \coordinate (Nz) at ($(N.west) + (0,\ioOffset)$);
     \coordinate (Ny) at ($(N.west) - (0,\ioOffset)$);

    % now link the nodes
%    \draw [connector] ($(Nu) + (1.5cm,0)$) -- node [pos=0.1, above] {$d$}
%                                                                node (Numid) [midway] {} (Nu);
%    \draw [connector] (Ny) -- node (Nymid) [midway] {}
%                                         node [pos=0.9, above] {$z$}($(Ny)-(1.5cm,0)$) ;

    \node (Numid) at ($(Nu) + (1.cm,0)$){};
    \node (Numid2) at ($(Numid) + (1.0cm,0)$){};
    \node (Nymid) at ($(Ny)-(1.cm,0)$){};
    \node (Nymid2) at ($(Nymid)-(1.5cm,0)$){};

    \draw [connector] (Nz) -- (Nz -| Nymid) |- (delta);
    \draw [connector]  (delta) -- (delta -| Numid) |- (Nv);

    \draw [connector] (Ny) -- (Ny -| Nymid2) |- (delta2);
    \draw [connector]  (delta2) -- (delta2 -| Numid2) |- (Nu);

    \path (N.north) -- node (midpoint) [midway]{} (delta.south) {};
    \path (N.north) -- node (midpoint2) [midway]{} (delta2.south) {};

    \node[left] at (Nymid |- midpoint) {$\zeta_1 = x$};
    \node[left] at (Nymid2 |- midpoint2) {$\zeta_2 = Tx + \mu y$};
%    \node[right] at (Numid2 |- midpoint2) {\phantom{$Tx + \mu y$}};
    \node[right] at (Numid |- midpoint) {$u_1$};
    \node[right] at (Numid2 |- midpoint2) {$u_2$\phantom{$= Tx + \mu y$}};

    \draw[red,ultra thick,dotted] ($(delta2.north west)+(-0.4,0.3)$)  rectangle ($(delta.south east)+(0.5,-0.2)$);
    \node [red] at ($(delta2.north east)+(0.3,0.0)$) {\large $\Delta$};


\end{tikzpicture} 

==> optalg2.tex <==
\input{Tikz_common_styles}%
\noindent%
%   set a filename for externalization
%\tikzsetnextfilename{clp_Ndelta_config}
%
\begin{tikzpicture}[scale=1, auto, >=stealth']

    \small

   % specify with respect to the plant

     \node[clpblock, minimum height=1.25cm, minimum width=1.25cm] (N)  {$G$};

     \node[deltablock, minimum height=1cm, minimum width=1cm, anchor=south, dotted]
                      (delta) at ($(N.north) + (0,0.35cm)$) {$\Delta$};

     \node[weightblock, minimum height=1cm, minimum width=1cm, anchor=south]
                      (psi) at ($(delta.north east) + (1.25cm,0.35cm)$) {$\Psi$};

     \def\ioOffset{0.25cm}
     \coordinate (Nv) at ($(N.east) + (0,\ioOffset)$);
     \coordinate (Nu) at ($(N.east) - (0,\ioOffset)$);
     \coordinate (Nz) at ($(N.west) + (0,\ioOffset)$);
     \coordinate (Ny) at ($(N.west) - (0,\ioOffset)$);
     
     \coordinate (Pzeta) at ($(psi.west) + (0,\ioOffset)$);
     \coordinate (Pu)    at ($(psi.west) - (0,\ioOffset)$);

    % now link the nodes
%    \draw [connector] ($(Nu) + (1.5cm,0)$) -- node [pos=0.1, above] {$d$}
%                                                                node (Numid) [midway] {} (Nu);
%    \draw [connector] (Ny) -- node (Nymid) [midway] {}
%                                         node [pos=0.9, above] {$z$}($(Ny)-(1.5cm,0)$) ;

    \node (Numid) at ($(Nu) + (1.cm,0)$){};
    \node (Nymid) at ($(Ny)-(1.cm,0)$){};
    
    \node (deltau) at ($(delta.east)+(.25cm,0)$){};
    \node (deltaz) at ($(delta.west)-(.5cm,0)$){};
    
    \node (psiout) at ($(psi.east)+(.5cm,0)$){$\eta$};

    \draw [connector] (delta.east) -| (deltau |- Pu) -- (Pu);
    \draw [connector] (delta.west) -| (deltaz |- Pzeta) -- (Pzeta);
    
    \draw [connector] (psi.east) -- (psiout);

    \draw [connector]  (N.west) -- (N.west -| Nymid) |- (delta);
    \draw [connector]  (delta.east) -- (delta -| Numid) |- (N.east);

    \path (N.north) -- node (midpoint) [midway]{} (delta.south) {};
    \path (N.north) -- node (midpoint2) [midway]{} (delta2.south) {};

    \node[left] at (Nymid |- midpoint) {$\zeta$};
    \node[right] at (Numid |- midpoint) {$u$};


\end{tikzpicture} 
